Low-complexity Multicast Beamforming for Multi-stream Multi-group Communications

In this paper, assuming multi-antenna transmitter and receivers, we consider multicast beamformer design for the weighted max-min-fairness (WMMF) problem in a multi-stream multi-group communication setup. Unlike the single-stream scenario, the WMMF objective in this setup is not equivalent to maximizing the minimum weighted SINR due to the summation over the rates of multiple streams. Therefore, the non-convex problem at hand is first approximated with a convex one and then solved using Karush-Kuhn-Tucker (KKT) conditions. Then, a practically appealing closed-form solution is derived, as a function of dual variables, for both transmit and receive beamformers. Finally, we use an iterative solution based on the sub-gradient method to solve for the mutually coupled and interdependent dual variables. The proposed solution does not rely on generic solvers and does not require any bisection loop for finding the achievable rate of various streams. As a result, it significantly outperforms the state-of-art in terms of computational cost and convergence speed.

==> conclusions.tex <==
%!TeX root = d2d-cc.tex
%\section{Discussion \& Future Work}
%\label{sec:discussion}

\section{Conclusions}
\label{sec:conclusions}
A novel delivery scheme optimized for finite \ac{SNR} region was proposed, where the multicast beamforming of file fragments is complemented by allowing direct \ac{D2D} exchange of local cache content. The benefits of partial D2D offloading of multicast delivery of coded caching content were investigated. Two straightforward example scenarios were assessed in details, and a generalized formulation was also provided. Moreover, we showed that using D2D transmission has two fold benefits. First, for appropriate D2D received SNR it will increase per user rate. Second, It will decrease the beamforming complexity by removing some terms from beamformer conditions which helps for less restricted and more powerful beams.
%We also provided two boundaries (for each of quadratic variables and MAC conditions) for general case (any $t, \ \text{and} \ L$) in order to better understand the role of D2D transmission in beam forming for downlink transmission.
 Moreover, we proposed a heuristic low complexity mode selection scheme with comparable performance to the optimal exhaustive search. We showed that using D2D greatly enhances the per-user rate and results in less restricted (less complex) beamforming problem. In future work, we are going to analyze the effects of D2D communication in energy efficiency of the network. %more realistic scenarios where the users experience different channel conditions in different groups.%Energy efficiency of the network is another perspective which will be covered in the future works.


%Furthermore, We investigate the effect of main parameters such as $t,\ L,\ \text{and} \ K$ in the per user rate, and showed that in general increasing $t$ will result in higher gain but increases D2D opportunity reduction with respect to user distance. On the other hand, increasing user number $K$ or $t+L$ increases the D2D opportunities and will result in higher gain.

==> systemmodel-old.tex <==
We consider a multi-group multicasting \ac{DL} scenario with $G$ different groups, $K$ single antenna users, and a single \ac{BS} equipped with $L$ antennas (as depicted in Fig.~\ref{fig:system-model}). Let us denote $ \mathcal{G} \triangleq \{1, 2, \dots, G\}$ as the set of all the group indices, and $\mathcal{K}_i \triangleq \{1, 2, \dots, K_i\}$ as the set of all the user indices within group $i \in \mathcal{G}$, where $\sum_{i \in \mathcal{G}}K_i = K$. The $L\times1$ channel vector between user $k$ and the \ac{BS} is denoted by ${\bf{h}}_{k} \sim \mathbb{CN}(0,\bf{I})$.  $L \times 1$ vector ${{\bf{w}}}_{i}$ denotes the transmit beamformer dedicated to group $i$, for $i \in \mathcal{G}$. The received signal at the user $k$ in group $i$ is given by
\begin{equation}
    y_{k} = {\mathbf h}_{k}^{\text{H}}{\bf w}_{i} x_{i} + \sum^{G}_{j \neq i}{\bf{h}}_{k}^{\text{H}}{{\bf{w}}}_{j} x_{j} + z_{k},
\end{equation}
 where $x_{i}$ is the dedicated message for group $i$ ($\mathbb{E} [|x_{i}|^2] =1$) and $z_{k}$ is an additive white Gaussian noise at user $k$, where $z_{k}\sim\mathbb{CN}(0, N_{0})$. The transmission power at the \ac{BS} is computed by $\sum_{i}^{G}\|{{\bf{w}}}_{i}\|^{2}$, and the received \ac{SINR} at the user $k$ in group $i$ is given by
 \begin{equation}
     \gamma_{i,k} = \frac{|{\bf{h}}_{k}^\text{H}{{\bf{w}}}_{i}|^2}{N_{0} + \sum^{G}_{j \neq i}|{\bf{h}}_{k}^{\text{H}}{{\bf{w}}}_{j}|^2}.
 \end{equation}
 
 \begin{figure}
    \centering 
    \includegraphics[width=0.9\columnwidth,keepaspectratio]{figs/sysmod.png}
    \caption{Multi-group multi-casting system model with $G = 3$ and $K = 9$.}
\label{fig:system-model}
\end{figure}
 
 \section{Problem formulation and solutions} \label{sec:prob-solu}
 
 In this paper, we consider max-min-fairness (\ac{MMF}) among all the users. In this regard, the aim is to maximize the minimum dedicated rate (or received \ac{SINR}) among all the users with respect to a limited total available power at the \ac{BS} ($P_{T}$). The optimization problem of the beamformer ${\bf{w}}_{i}$ is formulated as the following
\begin{equation}
\begin{aligned}
\label{eq:main-MMF}
\mathcal{S}_{0} \ : \quad \max_{\{{\bf{w}}_{i}\}, \gamma} \quad & \log(1+\gamma)\\
\textrm{s.t.} \quad & \gamma_{i,k} \geq \gamma, \quad  \forall k\in \mathcal{K}_i, \forall i\in\mathcal{G}, \\
& \sum_{i}^{G}\|{\bf{w}}_{i}\|^2 \leq P_{T}.
\end{aligned}
\end{equation}
Since the problem $\mathcal{S}_{0}$ is a well-known non-convex NP-hard problem\cite{MMF_QoS_MGMC_lefteris_2008}, the optimal solution is unattainable. However, There are different available numerical methods which aim to solve the problem in a sub-optimal manner such as \ac{SDR} and \ac{SCA}.The worst case complexity of the SDR is $\mathcal{O}(L^2 + K)^{3.5}$, whereas the complexity of the SCA is $\mathcal{O}(L + K)^{3.5}$ per-iteration, which make them impractical for large networks~\cite{MGMC-ADMM-based-fast-algorithm-2017}. In this paper, we aim to solve the \ac{MMF} problem in an iterative low complexity method which is based on \ac{KKT} conditions and sub-gradient method. For comparison we briefly explain the well-known SCA method~\cite{MGMC-SCA-ganesh-2017}, which we call \textit{Direct-SCA}. Motivated by the approach proposed in~\cite{MGMCmmf}, we also consider an alternative version of SCA, which we call \textit{Altered-SCA}, as a baseline.

It is worth mentioning that since logarithm is a monotonic function, from now on,  $\gamma$ (instead of $\log(1+\gamma)$) is considered as the objective function of $\mathcal{S}_{0}$.

 \subsection{Direct-SCA}
 
 The SINR constrains in $\mathcal{S}_{0}$ are not convex, however, they can be rewritten as the following~\cite{MGMC-SCA-ganesh-2017}
 %\begin{equation}
 \begin{align}
 &\gamma \leq   \frac{|{\bf{h}}_{k}^\text{H}{\bf{w}}_{i}|^2}{N_{0} + \sum^{G}_{j \neq i}|{\bf{h}}_{k}^{\text{H}}{\bf{w}}_{j}|^2}, \\
 &\Rightarrow N_{0} + \sum^{G}_{j \neq i}|{\bf{h}}_{k}^{\text{H}}{\bf{w}}_{j}|^2 
 \leq \frac{ |{\bf{h}}_{k}^{\text{H}}{\bf{w}}_{i}|^2}{\gamma} \label{eq:SINR-constrains}.
 \end{align}
 %\end{equation}
 
 Using the first order Taylor's approximation for the right hand side of~\eqref{eq:SINR-constrains}, the problem $\mathcal{S}_{0}$ can be written as follows
\begin{equation}
\begin{aligned}
\label{eq:direct-SCA-MMF}
&\mathcal{S}_{\text{sca}} \ : \quad \max_{\{{\bf{w}}_{i}\},\gamma} \quad  \gamma\\
&\textrm{s.t.} \quad  \sum_{j \neq i}|{\bf{w}}_{j}^{H}{\bf{h}}_{k}|^2 + N_{0} + \frac{|\overline{\bf{w}}_{i}^{H}{\bf{h}}_{k}|^2}{\Bar{\gamma}}(\frac{\gamma-\Bar{\gamma}}{\Bar{\gamma}}-1) \\
 & + \frac{2}{\Bar{\gamma}} \left(\R \left\{\overline{\bf{w}}_{i}^{H}{\bf{h}}_{k}{\bf{h}}_{k}^{H}(\overline{\bf{w}}_{i}-{\bf{w}}_{i})\right\}\right) \leq 0, \forall k\in \mathcal{K}_i, \forall i\in\mathcal{G},\\
& \sum_{i}^{G}\|{\bf{w}}_{i}\|^2 \leq P_{T},
\end{aligned}
\end{equation}
where $\overline{\bf{w}}_{j}$ and $\Bar{\gamma}$ are the previous beamformer and previous common \ac{SINR} from the last iteration, respectively. The problem $\mathcal{S}_{\text{sca}}$ is convex objective with convex constrains which can be efficiently solved with available generic solvers such as CVX. To solve $\mathcal{S}_{\text{sca}}$, we first initiate feasible beamformers $\overline{\bf{w}}_{i}^{0}$ and corresponding $\gamma^{0}$ for all the groups ($\forall i \in \mathcal{G}$) and solve $\gamma$ and ${\bf{w}}_{i}$ in $S_{\text{sca}}$. Next, $\overline{\bf{w}}_{i}$ and $\Bar{\gamma}$ are updated using the previously computed variables and solve the $S_{\text{sca}}$ again. The procedure is continued until the convergence.

Please note that in this approach, the complexity involved in each iteration of the SCA is proportional to the number of \ac{BS} antennas and the total number of users, i.e., $\mathcal{O}(L + K)^{3.5}$.

\subsection{Altered-SCA}

As an alternative approach, the authors in~\cite{MGMCmmf} have derived the Lagrangian dual problem for $\mathcal{S}_{\text{sca}}$, and approximated the dual variables $\lambda_{i,k}$  with the following iterative equation
\begin{equation}
\label{eq:iterative-gamma0}
    \Tilde{\lambda}_{i,k}^{l} = \frac{1}{(1+\gamma){\bf{h}}_{k}^{H}{\bf{A}}^{-1}({\Tilde{{\bf{\lambda}}}}^{l-1}){\bf{h}}_{k}}, \quad k \in \mathcal{K}_i,
\end{equation}
where $\Tilde{\lambda}_{i,k} = \frac{\lambda_{i,k}}{\mu}$ is the normalized dual variable, and $\lambda_{i,k}$ and $\mu$ are the Lagrangian dual variable for SINR and power constrains, respectively. Moreover, ${\Tilde{\lambda}}$ is defined as ${\Tilde{\lambda}} \triangleq [{\Tilde{\lambda}}^{T}_{1}, \dots, {\Tilde{\lambda}}^{T}_{G}]^{T}$ with ${\Tilde{\lambda}}_{i} \triangleq [\Tilde{\lambda}_{i,1}, \dots, \Tilde{\lambda}_{i,K_i}]^{T}$. Furthermore, ${\bf{A}}(\Tilde{\lambda})$ is a $L \times L$ matrix defined as ${\bf{A}}({\Tilde{\lambda}}) \triangleq \text{I} + \sum_{i \in G}\sum_{k \in \mathcal{K}_i}\Tilde{\lambda}_{i,k}{\bf{h}}_{k}{\bf{h}}_{k}^{H}$. After $\Tilde{\lambda}$ is converged to a stationary point (i.e., $\Tilde{\lambda}^{o}$), the beamformer is computed as ${\bf{w}}_{i}^{o} = {\bf{A}}^{-1}({\Tilde{\lambda}^{o}}){\bf{H}}_{i}{\bf{\zeta}}_{i}$, where ${\bf{H}}_{i} \triangleq [{\bf{h}}_{1}, \dots, {\bf{h}}_{K_i}]$. Finally, $K_i \times 1$ vectors $\{\zeta_{i}\}$ are computed through the following
 \begin{equation}
\begin{aligned}
\label{eq:main-MMF-degraded-sca}
\mathcal{S}_{\text{dsca}} \ : \quad & \min_{\{\zeta_{i}\}, \gamma} \quad  \gamma\\
\textrm{s.t.} \quad &  \frac{|{\zeta_{i}}^{H}{\bf{H}}_{i}^{H}{\bf{A}}^{-1}({\Tilde{\lambda}^{o}(\gamma)}){\bf{h}}_{k}|^2}{N_{0} + \sum^{G}_{j \neq i}|{\zeta_{j}^{o}}^{H}{\bf{H}}_{j}^{H}{\bf{A}}^{-1}({\Tilde{\lambda}^{o}(\gamma)}){\bf{h}}_{k}|^2} \geq \frac{1}{{\gamma}}, \\
&\quad  \forall k\in \mathcal{K}_i, \forall i\in\mathcal{G}, \\
& \sum_{i}^{G}\|{\zeta_{i}}^{H}{\bf{H}}_{i}^{H}{\bf{A}}^{-1}({\Tilde{\lambda}^{o}(\gamma)})\|^2 \leq P_{T}, \quad
 \gamma > 0.
\end{aligned}
\end{equation}

Note that the problem $\mathcal{S}_{\text{dsca}}$ is not convex and $\Tilde{\lambda}^{o}(\gamma)$ depends on the optimization variable $\gamma$. To tackle these issues, authors in~\cite{MGMCmmf} suggest to find the variable $\Tilde{\lambda}^{o}(\gamma)$ for a given $\gamma$ and then solve $\mathcal{S}_{\text{dsca}}$ as a feasibility problem with numerical methods (e.g., SCA). Also, variable $\gamma$ is found using bisection method such that the power constraint is met (please refer to~\cite{MGMCmmf} for more details). Note that compared to $\mathcal{S}_{\text{sca}}$, the size of the optimization variable has changed from $L \times 1$ vector ${\bf{w}}$ to $K_i \times 1$ vector $\zeta_i$  in $\mathcal{S}_{\text{dsca}}$, which makes it appealing for the large antenna regime $L \gg K_i$. In this regard, the complexity involved in solving $\mathcal{S}_{\text{dsca}}$ is $\mathcal{O}\left(K^{3.5}\right)$.

It is worth mentioning that though the problem $\mathcal{S}_{\text{dsca}}$ is independent from $L$, still $\Tilde{\lambda}^{o}(\gamma)$ and ${\bf{w}}_{i}^{o}$ depend on $L$ through the $L \times L$ matrix inversion. In this regard, the computation complexity of~\eqref{eq:iterative-gamma0} is approximately $\frac{2}{3}L^3 +2KL^2 +L +1$ flops per-iteration per user. Thus, assuming parallel computation for $\Tilde{\lambda}_{i,k}$ and ${\bf{w}}_{i}^{o}$, the complexity involved in this method is $\mathcal{O}(K^{3.5} + KL^2 + L^3)$ per-iteration. Also the computation complexity of ${\bf{w}}_{i}^{o}$ is approximately $\frac{2}{3}L^3 + KL^2 + 2L^{2}K_i+2LK_i$, which is done once after $\gamma$ and $\zeta$ are converged. Therefore, still there is a trade-off between the number of antenna at the base station and computational complexity of the method.

\subsection{Proposed iterative algorithm}

%Since the problem~\eqref{eq:direct-SCA-MMF} is convex, the solution for the primal problem and the dual problem is same. 
Denoting $\{\{{\bf{w}}_{i}\},\gamma\}$ as primal and $\{\lambda, \mu\}$ as dual variables, the Lagrange function for $\mathcal{S}_{\text{sca}}$ is formulated as the following
 \begin{equation}
     \begin{aligned}
     \label{eq:mmf-lagrangian}
     &\mathcal{L}(\lambda, {\bf{w}}, \overline{\bf{w}},\gamma,\Bar{\gamma}) = \frac{1}{\gamma} + \sum_{i \in \mathcal{G}}\sum_{k \in \mathcal{K}_i}\lambda_{i,k} \Bigg[\sum_{j \neq i}|{\bf{w}}_{j}^{H}{\bf{h}}_{k}|^2 \\
     & + \frac{|\overline{\bf{w}}_{i}^{H}{\bf{h}}_{k}|^2}{\Bar{\gamma}}(\frac{\gamma-\Bar{\gamma}}{\Bar{\gamma}}-1)
     + \frac{2}{\Bar{\gamma}}\Bigg(
     \R\big\{\overline{\bf{w}}_{i}^{H}{\bf{h}}_{k}{\bf{h}}_{k}^{H} \\ &(\overline{\bf{w}}_{i}-{\bf{w}}_{i})\big\}\Bigg) + N_{0} \Bigg] +   \mu(\sum_{i \in \mathcal{G}}\|{\bf{w}}_{i}\|^2-P_{T}).
     \end{aligned}
 \end{equation}
 
 Based on KKT conditions, the gradient of the Lagrangian function $\mathcal{L}(\lambda, {\bf{w}}, \overline{\bf{w}},\gamma)$ with respect to primal variables (i.e., $\{\{{\bf{w}}_{i}\},\gamma\}$) must vanish at the optimal point. Therefore, for a given $\Bar{\gamma}$ and $\overline{\bf{w}}$, the beamformer structure and the common SINR are formulated as
   \begin{equation}
     \begin{aligned}
     \label{eq:lagrangian-beamformer structure-MMF}
     &\nabla_{{\bf{w}}_{i}}\mathcal{L}(\lambda, {\bf{w}}, \overline{\bf{w}},\mu, \Bar{\gamma})=0 \Rightarrow {\bf{w}}_{i}^{*} = \Psi_{-i}^{-1}(\lambda^{*}, \mu^{*})\Phi_{i}(\lambda^{*}, \overline{\bf{w}}_{i}), \\
     &\nabla_{\gamma}\mathcal{L}(\lambda, {\bf{w}}, \overline{\bf{w}},\mu, \Bar{\gamma})=0 \Rightarrow  \\
     &\gamma^{*} = \sqrt{\frac{\Bar{\gamma}^2}{\sum_{i \in \mathcal{G}}\sum_{k \in \mathcal{K}_i}\lambda_{i,k}^{*}|\overline{\bf{w}}_{i}^{H}{\bf{h}}_{k}|^2}},
     \end{aligned}
 \end{equation}
 where $\Psi_{-i}(\lambda^{*}, \mu^{*}) \triangleq \left(\mu^{*}{\bf{I}} + \sum_{j \neq i}\sum_{k \in \mathcal{K}_j}\lambda_{j,k}^{*}{\bf{h}}_{k}{\bf{h}}_{k}^{H}\right)$, $\mu^{*}$ and $\lambda^{*}_{i,k}$ are the optimal dual variables for power constrains and SINR constrains, respectively. Denote $\Phi_{i}(\lambda^{*}, \overline{\bf{w}}_{i}) \triangleq \frac{1}{\Bar{\gamma}}\left(\sum_{k \in \mathcal{K}_i}\lambda_{i,k}^{*}\overline{\bf{w}}_{i}^{H}{\bf{h}}_{k}{\bf{h}}_{k}\right)$ as the weighted users' channel effect in the $i$'th beamformer. Considering~\eqref{eq:lagrangian-beamformer structure-MMF}, it can be shown that the optimal beamformer (for a given $\overline{\bf{w}}$) has weighted MMSE structure~\cite{MGMCmmf}. The dual variables in~\eqref{eq:mmf-lagrangian} are highly coupled; therefore, finding them directly from KKT conditions is unattainable. In the following, we propose iterative equations to update the dual and primal variables in each step based on the variables from the previous step until convergence
    \begin{subequations}
     \begin{align}
     &{\bf{w}}_{i}^{l} = \Psi_{-i}^{-1}(\lambda^{l-1}, \mu^{l})\Phi_{i}(\lambda^{l-1}, {\bf{w}}_{i}^{l-1}), \label{eq:itw0-mmf} \\
     %&{\bf{w}}_{i}^{l} = {\bf{w}}_{i}^{l-1} + \alpha({\bf{w}}_{i}^{o} - {\bf{w}}_{i}^{l-1}),\label{eq:itwl-mmf} \\
     &\gamma_{i,k}^{l} = \frac{|{\bf{h}}_{k}^\text{H}{\bf{w}}_{i}^{l}|^2}{N_{0} + \sum^{G}_{j \neq i}|{\bf{h}}_{k}^{\text{H}}{\bf{w}}_{j}^{l}|^2}, \label{eq:itgamal-mmf}\\
     &\gamma^{l} =  \sqrt{\frac{({\gamma}^{l-1})^2}{\sum_{i \in \mathcal{G}}\sum_{k \in \mathcal{K}}\lambda_{i,k}^{l-1}|{\bf{h}}_{k}^{H}{{\bf{w}}_{i}^{l-1}}|^2}}, \label{eq:itgamma0-mmf} \\
     %&\gamma^{l} = \gamma^{l-1} + \varphi(\gamma^{o}-\gamma^{l-1}), \label{eq:itcgammal-mmf} \\
     &\lambda_{i,k}^{l} = \big(\lambda_{i,k}^{l-1} + \beta(\gamma^{l}-\gamma_{i,k}^{l})\big)^{+},\label{eq:itlambda-mmf}
     \end{align}
 \end{subequations}
  where $(x)^{+} \triangleq \text{max}(0,x) $, and $\beta > 0$ is the step size for dual variable updates. Thus, KKT conditions for \eqref{eq:mmf-lagrangian} are solved iteratively, starting with some random initial points $\{{\bf{w}}^{0}, \ \lambda^{0}, \gamma^{0}\}$ \footnote{It can be shown that with an appropriate step size, the algorithm converges to the optimal point with any random initial points, provided that enough number of iterations are allowed.}. The dual variable $\mu^{l}$ (in each iteration) is computed by bisection method such that the power constraint in~\eqref{eq:mmf-lagrangian} is met. Please note that the dual variables $\{\lambda^{l}_{i,k}\}$ are updated through~\eqref{eq:itlambda-mmf} using the sub-gradient method without relying on any generic solvers. Finally, the complete process of the proposed iterative update of the primal and the dual variables is summarized in Algorithm~\ref{algorithm:MMF}.
  
  Note that in~\eqref{eq:itw0-mmf}, the beamformer ${\bf{w}}^{l}_{i}$ is independent of other beamformers and only depends on variables from previous iterations. Thus, all the beamformers can be updated in parallel, which reduces the execution time compared to generic solvers (which attempt to solve all the beamformers jointly). Moreover, in~\eqref{eq:itgamma0-mmf}, we approximate the potential common SINR based on the previous beamformers, and in~\eqref{eq:itlambda-mmf}, we check whether the received SINR of user $k$ in group $i$ is equal to $\gamma^{l}$ or not. If the received SINR of a particular user is less than the approximated common SINR, we increase the user's channel effect (i.e., $\lambda_{i,k}$) in the beamformers through~\eqref{eq:itlambda-mmf}, and if its higher than $\gamma^{l}$ we decrease the effect. In general, in each iteration, the beamformer ${\bf{w}}^{l}_{i}$ turns in the direction of the channel of the user with the lowest received SINR in $\mathcal{K}_i$. Thus, in the next iteration, $\overline{\bf{w}}_{i}$ and ${\bf{h}}_{k}$ have a higher inner product, which leads to SINR improvement of that user.
  
The complexity of the proposed algorithm is dominated by the $L \times L$ matrix inversion in~\eqref{eq:itw0-mmf}. In this regard, the computation complexity to create $\Psi_{-i}^{-1}$ is approximately $KL^2 + \frac{2}{3}L^3$ flops. Moreover, the computation complexity to create $\Psi_{-i}^{-1}\Phi_{i}$ is $3LK_i + L^2$ flops. Thus, in general the complexity of the proposed method is $\mathcal{O}(KL^2+L^3)$ per-iteration, assuming parallel beamforming updates. For a moderate number of antennas, the proposed algorithm converges to the stationary point quickly and significantly faster than the other two approaches above. It is worth mentioning that for the particular case of coded caching, the number of antennas and the number of users are typically within the same range, which makes the proposed algorithm appealing for the CC. 
 
 \begin{algorithm}
\SetAlgoLined
\KwResult{${\bf{w}}_{i}, \lambda_{i,k}$, $\gamma$}
initialization\; 
 set $l =1$ and choose any random variables for \{${\bf{w}}_{i}^{0}$, $\lambda_{i,k}^{0}, \gamma^{0}\},  \forall k \in \mathcal{K}_i$, and $\forall i \in \mathcal{G}$\; 
 \While{ $l \leq$ {ITERATION} {\bf or} until convergence}{
  compute $\mu^{l}$ using bisection such that $\sum_{i \in \mathcal{G}}\|{\bf{w}}_{i}^{l}\|^2 \leq P_{T}$; 
  
 solve ${\bf{w}}_{i}^{l}$ from~\eqref{eq:itw0-mmf} using $\{{\bf{w}}_{i}^{l-1},\lambda^{l-1}, \mu^{l}\}$ ; 
 
  %update ${\bf{w}}_{i}^{l}$ from~\eqref{eq:itwl-mmf} based on $\{{\bf{w}}_{i}^{o},{\bf{w}}_{i}^{l-1}\}$ ;
  
  compute $\gamma^{l}$ from~\eqref{eq:itgamma0-mmf} using $\{\{{\bf{w}}_{i}^{l-1}\}, \gamma^{l-1}$\} ;
  
  %update $\gamma^{l}$ from~\eqref{eq:itcgammal-mmf} using $\{\gamma^{o}, \gamma^{l-1}\}$ ;
  
  compute $\gamma_{i,k}^{l}$ from~\eqref{eq:itw0-mmf} using \{${\bf{w}}_{i}^{l}$\} ;
  
  update $\lambda_{i,k}^{l}$ from~\eqref{eq:itlambda-mmf} using  $\{\gamma_{i,k}^{l-1}, \gamma_{i,k}^{l},{\gamma}^{l}\}$ ;
  
  $l= l+1$ ;

 }
 \caption{Low complexity iterative algorithm for max-min-fairness problem}
 \label{algorithm:MMF}
\end{algorithm}


%%%%%%%% simulations %%%%%%%%%%%%%%%%%%%%%%%%

To evaluate the proposed algorithm, we have performed simulations and compared the three methods as mentioned earlier, considering the computation time and the output results. We consider \ac{DL} system with $K_i= \overline{K} = 5, \ \forall i \in \mathcal{G}$, $G=3$ and $N_{0} = 1$. The step size $\beta$ is variable between $[10^{-5} \quad 10^{-2}]$, based on the number of antennas (on average $\beta \approx 10^{-3}$). The available power at the \ac{BS} is $5$ dB (i.e., $P_{T}=5$ dB).

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table}[t]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}The number of \\ antennas L\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Proposed \\ iterative\\ algorithm\end{tabular} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Altered\\ SCA\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Direct\\ SCA\end{tabular} \\ \cline{3-4}& &$\mathcal{S}_{\text{dsca}}$& $\tilde{\lambda}_{i,k}$ & \\ \hline
30  & 0.054 &  1.4  & $\leq$ 0.03  & 1.5 \\50  & 0.072  &  1.4  & $\leq$ 0.03  & 1.7 \\ 70  & 0.111 &  1.4  & $\leq$ 0.05  & 1.9 \\ 85  & 0.135 &  1.4 & $\leq$ 0.07& 2 \\ 100  & 0.165 & 1.4  & $\leq$ 0.07 & 2\\ \hline
\end{tabular}
\vspace{1mm}
\caption{Average computation time per-iteration for a fixed $\overline{K}=5$ users within each group}
\label{table:mmf}
\end{table}

\begin{table}[t]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}The number of \\ users within \\ each group $\overline{K}$\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Proposed \\ iterative\\ algorithm\end{tabular} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Altered\\ SCA\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Direct\\ SCA\end{tabular} \\ \cline{3-4}& &$\mathcal{S}_{\text{dsca}}$& $\tilde{\lambda}_{i,k}$ & \\ \hline
5  & 0.063 &  1.4  & $\leq$ 0.03  & 1.7 \\10  & 0.075  &  2.4  & $\leq$ 0.03  & 2.1 \\ 15  & 0.087 &  3.4  & $\leq$ 0.03  & 2.8 \\ 20  & 0.105 &  4.5 & $\leq$ 0.03& 3.4 \\ \hline
\end{tabular}
\vspace{1mm}
\caption{Average computation time per-iteration for a fixed $L=50$ antennas at the BS}
\label{tab:mmfk}
\end{table}

\begin{table}[t] 
\centering
\begin{tabular}{|l|l|l|l|}
\hline
 $\ \ \ \Biggm\backslash$   & \begin{tabular}[c]{@{}l@{}} Per-iteration Complexity\end{tabular} & \begin{tabular}[c]{@{}l@{}}Average \\ number of\\  iterations\end{tabular} & \begin{tabular}[c]{@{}l@{}}Overall\\ computation \\ time\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Direct\\ SCA\end{tabular}& $\mathcal{O}\left((L + K)^{3.5}\right)$ & $\leq 100$ & medium \\ \hline \begin{tabular}[c]{@{}l@{}}Altered\\ SCA\end{tabular}& $\mathcal{O}\left(K^{3.5} + (K+L)L^2\right)$ & $\leq 100$ & low \\ \hline \begin{tabular}[c]{@{}l@{}}Proposed\\ method\end{tabular} & $\mathcal{O}\left((K+L)L^2\right)$& $\leq 100$ & very low \\ 
\hline
\end{tabular} 
\vspace{1mm}
\caption{Overall performance comparison}
\label{table: overal performance}
\end{table}

\begin{figure}
    \centering 
    \includegraphics[width=0.8\columnwidth,keepaspectratio]{figs/RSNR.eps}
    \caption{Maximum common SINR Vs. the number of antenna $L_g$ at the base station for $\overline{K}=5, \ G=3, \ P_{T}=5$dB.}
\label{fig:sinr-mmf}
\end{figure}

\begin{figure}
    \centering 
    \includegraphics[width=0.8\columnwidth,keepaspectratio]{figs/KSNR.eps}
    \caption{Maximum common SINR Vs. the number of users $\overline{K}$ within each group for $L=50, \ G=3, \ P_{T}=5$dB.}
\label{fig:ksinr-mmf}
\end{figure}

Fig.~\ref{fig:sinr-mmf} compares the maximum common rate against the number of antennas at the \ac{BS} for the three methods. As illustrated, the proposed method provides the same favorable performance as the other state of the arts (SoA) with significantly lower computation time and complexity. Table~\ref{table:mmf} compares the computation time per-iteration for the three methods. Since many parameters, such as step size, initial point, CVX accuracy, etc. affects the total computation time and convergence rate, the average simulation time per-iteration is being compared.

Fig.~\ref{fig:ksinr-mmf} shows the maximum common SINR versus the number of users within each group. As depicted, the same favorable performance is achieved by the proposed method with much lower computation time and complexity compared to the "\textit{Altered-SCA}" and "\textit{Direct-SCA}". The average per-iteration computation time for Fig.~\ref{fig:ksinr-mmf} is shown in Table~\ref{tab:mmfk}. It is worth to mention that when the total number of users (i.e., $G\overline{K} = K$) increases to the same range as the number of BS antennas, the computation complexity difference between the proposed method and other approaches is more noticeable. As a result, when the total number of antennas and the total number of users are within the same range, the proposed algorithm outperforms the existing methods in the sense of computation time and complexity. Finally, Table~\ref{table: overal performance} compares the overall performance of the three methods.

